Large-time behavior of finite-state mean-field systems with multi-classes

We study in this paper the large-time asymptotics of the empirical vector associated with a family of finite-state mean-field systems with multi-classes. The empirical vector is composed of local empirical measures characterizing the different classes within the system. As the number of particles in the system goes to infinity, the empirical vector process converges towards the solution to a McKean-Vlasov system. First, we investigate the large deviations principles of the invariant distribution from the limiting McKean-Vlasov system. Then, we examine the metastable phenomena arising at a large scale and large time. Finally, we estimate the rate of convergence of the empirical vector process to its invariant measure. Given the local homogeneity in the system, our results are established in a product space.

==> babelbst.tex <==
%%
%% This is file `merlin.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from merlin.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
%\ifcase\language \input{frenbst} \or \input{frenbst}
%\else \input{frenbst} \fi
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{r\'edacteurs}        \def\bbleds{r\'ed.}
\def\bbleditor{r\'edacteur}          \def\bbled{r\'ed.}
\def\bbledby{edit\'e par}
\def\bbledition{edition}        \def\bbledn{ed}
\def\bblvolume{tome}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n$^\mathrm{o}$}
\def\bblin{dans}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Rapport technique}
\def\bbltechrep{Rap. Tech.}
\def\bblmthesis{Th\`ese de ma\^itre}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1ere}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\`eme}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\`eme}
\def\bblfourth{Quatri\`eme}          \def\bblfourtho{4\`eme}
\def\bblfifth{Cinqui\`eme}            \def\bblfiftho{5\`eme}
\def\bblst{$^{\mbox{\scriptsize \`ere}}$}  
\def\bblnd{$^{\mbox{\scriptsize \`eme}}$}  
\def\bblrd{$^{\mbox{\scriptsize \`eme}}$}
\def\bblth{$^{\mbox{\scriptsize \`eme}}$}
\def\bbljan{janvier}  \def\bblfeb{f\'evrier}  \def\bblmar{mars}
\def\bblapr{avril}    \def\bblmay{mai}       \def\bbljun{juin}
\def\bbljul{juillet}     \def\bblaug{ao\^ut}    \def\bblsep{septembre}
\def\bbloct{octobre}  \def\bblnov{novembre}  \def\bbldec{d\'ecembre}
\endinput
%%
%% End of file `merlin.tex'.

